Towards Reasoning Ability of Small Language Models

Reasoning has long been viewed as an emergent property of large language models (LLMs). However, recent studies challenge this assumption, showing that small language models (SLMs) can also achieve competitive reasoning performance. This paper introduces ThinkSLM, the first extensive benchmark to systematically evaluate and study the reasoning abilities of SLMs trained from scratch or derived from LLMs through quantization, pruning, and distillation. We first establish a reliable evaluation criterion comparing available methods and LLM judges against our human evaluations. Then we present a study evaluating 72 diverse SLMs from six major model families across 17 reasoning benchmarks. We repeat all our experiments three times to ensure a robust assessment. Our findings show that: 1) reasoning ability in SLMs is strongly influenced by training methods and data quality rather than solely model scale; 2) quantization preserves reasoning capability, while pruning significantly disrupts it; 3) larger models consistently exhibit higher robustness against adversarial perturbations and intermediate reasoning, but certain smaller models closely match or exceed the larger models' performance. Our findings challenge the assumption that scaling is the only way to achieve strong reasoning. Instead, we foresee a future where SLMs with strong reasoning capabilities can be developed through structured training or post-training compression. Our ThinkSLM Leaderboard is publicly available at: https://ctrl-gaurav.github.io/thinkslm.github.io/

==> tikzlibraryshapes.emoticon.code.tex <==
%
%
%
\pgfdeclareshape{emoticon happy}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
    \pgfpathellipse{\pgfqpoint{-.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
                          \pgfusepath{stroke}%
\begingroup
\pgfsetlinewidth{0.4pt}%
\pgflowlevelsynccm    
       \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
      \pgfpatharc{-135}{-45}{.5\pgfutil@tempdima and .5\pgfutil@tempdima}%
      \pgfusepath{stroke}%
\endgroup    
  }} 

  \pgfdeclareshape{emoticon sad}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
    \pgfpathellipse{\pgfqpoint{-.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
                          \pgfusepath{stroke}%
\begingroup
\pgfsetlinewidth{0.4pt}%
\pgflowlevelsynccm    
      \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
 \pgfpathcurveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}
                {\pgfpoint{0pt}{-.153\pgfutil@tempdima}}
                {\pgfqpoint{.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}
      \pgfusepath{stroke}%
\endgroup    
  }}  

    \pgfdeclareshape{emoticon straight face}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
    \pgfpathellipse{\pgfqpoint{-.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
                          \pgfusepath{stroke}%
\begingroup
  \pgfsetlinewidth{0.4pt}%
  \pgflowlevelsynccm    
  \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
  \pgfpathlineto{\pgfqpoint{.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}
  \pgfusepath{stroke}%
\endgroup    
  }}  
      \pgfdeclareshape{emoticon wink}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathmoveto{\pgfqpoint{-.40\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
    \pgfpathcurveto{\pgfqpoint{-.40\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                {\pgfqpoint{-.25\pgfutil@tempdima}{.10\pgfutil@tempdima}}%
                {\pgfqpoint{-.10\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
    \pgfusepath{fill}%
    \pgfusepath{stroke}%
\begingroup
   \pgfsetlinewidth{0.4pt}%
   \pgflowlevelsynccm    
   \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
   \pgfpatharc{-135}{-45}{.5\pgfutil@tempdima and .5\pgfutil@tempdima}%
   \pgfusepath{stroke}%
\endgroup      
  }}%
\endinput
